Adapting Large Language Models for Document-Level Machine Translation

Large language models (LLMs) have significantly advanced various natural language processing (NLP) tasks. Recent research indicates that moderately-sized LLMs often outperform larger ones after task-specific fine-tuning. This study focuses on adapting LLMs for document-level machine translation (DocMT) for specific language pairs. We first investigate the impact of prompt strategies on translation performance and then conduct extensive experiments using two fine-tuning methods, three LLM backbones, and 18 translation tasks across nine language pairs. Our results show that specialized models can sometimes surpass GPT-4 in translation performance but still face issues like off-target translation due to error propagation in decoding. We provide an in-depth analysis of these LLMs tailored for DocMT, examining translation errors, discourse phenomena, strategies for training and inference, the data efficiency of parallel documents, recent test set evaluations, and zero-shot crosslingual transfer. Our findings highlight the strengths and limitations of LLM-based DocMT models and provide a foundation for future research.

==> 7_discussion.tex <==
\section{Discussion}

\paragraph{Evaluation}


\paragraph{Prompting Strategy}


\paragraph{Low-Resource Languages}

==> figures/elo_prompt.tex <==

\begin{figure*}[t]
    \centering
    \footnotesize
    \begin{Verbatim}[frame=single, fontsize=\footnotesize, breaklines=true, breakanywhere=true, commandchars=\\\{\}]
[Context]:
[<src_lang>]: <src1> <src2> <src3>
[<tgt_lang>]: <tgt1> <tgt2> <tgt3>

[Source]:
[<src_lang>]: <src4>

[Reference]:
[<tgt_lang>]: <tgt4>

[Assistant 1's Translation]:
[<tgt_lang>]: <hyp4_asst1>

[Assistant 2's Translation]:
[<tgt_lang>]: <hyp4_asst2>

We would like to request your feedback on the translation quality from <src_lang> to <tgt_lan> provided by two AI assistants. Please determine which translation is better and justify your choice. Pay extra attention to how the translations relate to their context. Return "1" if the translation provided by Assistant 1 is better, "2" if that by Assistant 2 is better, and "0" if they are equally good or bad.
    \end{Verbatim}
    \caption{Prompt used for \elo ratings.}
    \label{fig:elo_prompt}
\end{figure*}

==> figures/radars_en_x.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[scale=0.6]{assets/radars_en_x.pdf}
    \caption{
    Breakdown results on \sbleu, \dbleu, and \comet given by \oursllamasmalllora, \oursvicunasmalllora, \oursbloomsmalllora, \docnmtmtfivelarge, and \gptfour for the translation tasks \textbf{from English to other languages}.
    % \trang{Interestingly, L-7B-LoRA and V-7B-LoRA are almost always on par, except for de, fr and it. It might be related to our conclusion in section 6.3 that the second step (finetuning on parallel data) is mainly for activate the inherent translation capabilities. If this hypothesis is true, the two models should have similar performance. Any speculation on the discrepancy in the cases of de, fr and it? }
    }
    \label{fig:radars_en_x}
\end{figure*}

==> tables/elo_en_x.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{lccccccccc}
\toprule
                     & Ar             & De             & Fr             & It             & Ja             & Ko             & Nl             & Ro             & Zh             \\ \midrule
\nllbsmall           & 1070           & 1090           & 1113           & 1184           & 1036           & 1105           & 1213           & 1126           & \phantom{0}973 \\
\nllbmedium          & 1143           & 1194           & 1169           & 1234           & 1045           & 1204           & 1261           & 1191           & \phantom{0}908 \\
\nllbbig             & 1201           & 1197           & 1201           & 1286           & 1127           & 1164           & 1310           & 1211           & \phantom{0}947 \\
\googletrans         & 1079           & 1087           & 1128           & 1250           & 1166           & 1048           & 1254           & 1100           & 1031           \\ \midrule
\chatgpt             & 1166           & 1230           & 1264           & 1315           & 1291           & 1173           & 1346           & 1256           & 1192           \\
\gptfour             & 1262           & 1296           & 1286           & 1343           & 1353           & 1340           & 1421           & 1314           & 1262           \\ \midrule
\model{Llama2-7B}    & \phantom{0}564 & \phantom{0}820 & \phantom{0}729 & \phantom{0}776 & \phantom{0}760 & \phantom{0}829 & \phantom{0}699 & \phantom{0}701 & \phantom{0}917 \\
\model{Bloom-7B}     & \phantom{0}760 & \phantom{0}699 & 1025           & \phantom{0}706 & \phantom{0}650 & \phantom{0}590 & \phantom{0}764 & \phantom{0}515 & \phantom{0}724 \\
\model{Vicuna-7B}    & \phantom{0}759 & \phantom{0}780 & \phantom{0}678 & \phantom{0}857 & 1130           & 1037           & \phantom{0}958 & \phantom{0}802 & 1086           \\ \midrule
\docnmtmtfivesmall   & \phantom{0}864 & \phantom{0}783 & \phantom{0}818 & \phantom{0}961 & \phantom{0}972 & \phantom{0}950 & \phantom{0}943 & \phantom{0}837 & \phantom{0}921 \\
\docnmtmtfivebase    & \phantom{0}989 & \phantom{0}893 & \phantom{0}896 & 1000           & 1078           & 1080           & \phantom{0}972 & \phantom{0}890 & 1015           \\
\docnmtmtfivelarge   & \phantom{0}953 & \phantom{0}926 & \phantom{0}894 & 1007           & 1119           & 1031           & \phantom{0}962 & \phantom{0}949 & 1018           \\ \midrule
\oursllamasmalllora  & 1036           & 1093           & 1071           & \phantom{0}771 & 1025           & 1046           & \phantom{0}732 & 1128           & 1082           \\
\oursllamasmallfft   & 1108           & 1121           & \phantom{0}822 & \phantom{0}723 & \phantom{0}966 & \phantom{0}964 & \phantom{0}736 & 1108           & 1002           \\
\oursbloomsmalllora  & \phantom{0}967 & \phantom{0}912 & 1058           & 1113           & \phantom{0}742 & \phantom{0}633 & 1120           & \phantom{0}823 & \phantom{0}942 \\
\oursbloomsmallfft   & \phantom{0}950 & \phantom{0}910 & 1123           & \phantom{0}804 & \phantom{0}673 & \phantom{0}616 & \phantom{0}845 & \phantom{0}957 & \phantom{0}851 \\
\oursvicunasmalllora & 1064           & \phantom{0}948 & \phantom{0}882 & \phantom{0}917 & 1030           & 1059           & \phantom{0}781 & 1116           & 1111           \\
\oursvicunasmallfft  & 1066           & 1022           & \phantom{0}843 & \phantom{0}753 & \phantom{0}837 & 1130           & \phantom{0}686 & \phantom{0}976 & 1020           \\ \bottomrule
\end{tabular}
\caption{Breakdown \elo results for the translation tasks from English to other languages.}
\label{tab:elo_en_x}
\end{table*}

==> tables/elo_x_en.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{lccccccccc}
\toprule
                     & Ar             & De             & Fr             & It             & Ja             & Ko             & Nl             & Ro             & Zh             \\ \midrule
\nllbsmall           & 1006           & \phantom{0}720 & \phantom{0}867 & \phantom{0}791 & 1049           & 1108           & \phantom{0}735 & \phantom{0}723 & 1055           \\
\nllbmedium          & 1182           & \phantom{0}859 & 1004           & \phantom{0}913 & 1082           & 1143           & \phantom{0}891 & \phantom{0}844 & 1092           \\
\nllbbig             & 1141           & \phantom{0}926 & 1001           & \phantom{0}980 & 1096           & 1267           & \phantom{0}909 & \phantom{0}909 & 1060           \\
\googletrans         & 1172           & 1078           & 1010           & 1003           & 1124           & 1154           & 1057           & 1057           & 1062           \\ \midrule
\chatgpt             & 1318           & 1223           & 1194           & 1220           & 1405           & 1351           & 1199           & 1235           & 1364           \\
\gptfour             & 1352           & 1254           & 1199           & 1205           & 1446           & 1411           & 1207           & 1291           & 1394           \\ \midrule
\model{Llama2-7B}    & \phantom{0}803 & \phantom{0}803 & \phantom{0}690 & \phantom{0}989 & \phantom{0}798 & \phantom{0}832 & 1069           & \phantom{0}844 & \phantom{0}859 \\
\model{Bloom-7B}     & \phantom{0}972 & \phantom{0}873 & 1011           & \phantom{0}942 & \phantom{0}734 & \phantom{0}734 & \phantom{0}718 & \phantom{0}659 & \phantom{0}657 \\
\model{Vicuna-7B}    & \phantom{0}798 & \phantom{0}913 & \phantom{0}944 & \phantom{0}809 & 1014           & \phantom{0}821 & \phantom{0}901 & \phantom{0}739 & \phantom{0}933 \\ \midrule
\docnmtmtfivesmall   & \phantom{0}890 & \phantom{0}832 & \phantom{0}787 & \phantom{0}793 & \phantom{0}964 & \phantom{0}960 & \phantom{0}774 & \phantom{0}799 & \phantom{0}952 \\
\docnmtmtfivebase    & \phantom{0}988 & \phantom{0}884 & \phantom{0}832 & \phantom{0}870 & 1026           & 1050           & \phantom{0}831 & \phantom{0}856 & 1000           \\
\docnmtmtfivelarge   & 1036           & \phantom{0}874 & \phantom{0}806 & \phantom{0}824 & 1055           & 1022           & \phantom{0}894 & \phantom{0}906 & 1026           \\ \midrule
\oursllamasmalllora  & \phantom{0}821 & 1172           & 1093           & 1125           & \phantom{0}889 & \phantom{0}836 & 1171           & 1231           & \phantom{0}894 \\
\oursllamasmallfft   & \phantom{0}799 & 1128           & 1111           & 1165           & \phantom{0}846 & \phantom{0}802 & 1161           & 1212           & \phantom{0}892 \\
\oursbloomsmalllora  & 1134           & 1102           & 1107           & 1131           & 1051           & 1055           & 1073           & 1142           & 1227           \\
\oursbloomsmallfft   & \phantom{0}914 & 1075           & 1105           & 1100           & \phantom{0}772 & \phantom{0}752 & 1073           & 1136           & \phantom{0}778 \\
\oursvicunasmalllora & \phantom{0}840 & 1128           & 1102           & \phantom{0}964 & \phantom{0}790 & \phantom{0}869 & 1181           & 1225           & \phantom{0}877 \\
\oursvicunasmallfft  & \phantom{0}833 & 1156           & 1138           & 1175           & \phantom{0}859 & \phantom{0}832 & 1155           & 1192           & \phantom{0}877 \\ \bottomrule
\end{tabular}
\caption{Breakdown \elo results for the translation tasks from other languages to English.}
\label{tab:elo_x_en}
\end{table*}

==> tables/zero_shot_lite.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{6pt}
\begin{tabular}{lccccc}
\toprule
                     & $\mu_{\Delta}$ & Ar    & De    & Fr    & Zh    \\ \toprule
\oursllamasmalllora  & +29.4          & +36.3 & +38.8 & +37.2 & +29.5 \\
\oursllamasmallfft   & +29.0          & +41.2 & +40.5 & +37.1 & +37.5 \\
\oursbloomsmalllora  & +20.3          & \phantom{0}+7.5  & +40.7 & +20.7 & \phantom{0}+9.8  \\
\oursbloomsmallfft   & +27.3          & +14.8 & +37.8 & +28.9 & +19.5 \\
\oursvicunasmalllora & \phantom{0}-8.9           & -12.6 & +22.1 & +18.9 & -34.1 \\
\oursvicunasmallfft  & \phantom{0}-1.4           & \phantom{0}+7.3  & +25.2 & +17.7 & \phantom{0}-3.5  \\ \bottomrule
\end{tabular}
\caption{
The difference ($\Delta$) in \comet scores on the test sets from English to other languages between our English-German LLM-based \docnmt models and their backbones. $\mu_{\Delta}$ indicates the average difference across all the languages in this table.
The complete results are presented in \autoref{sec:transfer}.
}
\label{tab:zero_shot_lite}
\end{table}

